Partial Selfish Mining for More Profits

Mining attacks aim to gain an unfair share of extra rewards in the blockchain mining. Selfish mining can preserve discovered blocks and strategically release them, wasting honest miners' computing resources and getting higher profits. Previous mining attacks either conceal the mined whole blocks (hiding or discarding), or release them completely in a particular time slot (e.g., causing a fork). In this paper, we extend the mining attack's strategy space to partial block sharing, and propose a new and feasible Partial Selfish Mining (PSM) attack. We show that by releasing partial block data publicly and attracting rational miners to work on attacker's private branch, attackers and these attracted miners can gain an unfair share of mining rewards. We then propose Advanced PSM (A-PSM) attack that can further improve attackers' profits to be no less than the selfish mining. Both theoretical and experimental results show that PSM attackers can be more profitable than selfish miners under a certain range of mining power and network conditions. A-PSM attackers can gain even higher profits than both selfish mining and honest mining with attracted rational miners.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	ccs-template.tex 

PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf}

all:  ${PDF}

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'


==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> cfp.tex <==
\section{Call for Papers}

The conference seeks submissions presenting novel research results in
all aspects of computer and communications security and privacy,
including both practical and theoretical contributions.

\subsection{Paper Submission Information}

Submissions must be received at \url{https://ccs17.hotcrp.com/} by the
strict deadline of {\bf 19 May 2017 at 8:59 PM PDT (UTC-7)}.
Submitted papers must not substantially overlap with papers that have
been published or that are simultaneously submitted to a journal,
conference, or workshop. Submissions must be anonymized and avoid
obvious self-references.

CCS has traditionally required that authors submitting papers
guarantee that an author will be able to present their paper at the
conference. We recognize, however, that the current travel
restrictions and screening processes may make it impossible or
uncomfortable for some authors to travel to the conference. The venue
for CCS 2017 was selected several years ago, and we do not wish to
exclude any potential authors who may have difficulty traveling due to
recent changes in US immigration practices.  CCS welcomes submissions
by authors of all nationalities, and will make allowances for
presenting papers electronically or with non-author presenters in
cases where paper authors are unable to travel to the United States.

Submissions will be evaluated based on their scientific merit,
novelty, importance, presentation quality, and relevance to computer
and communications security and privacy.  If a paper includes work
that raises ethical concerns it is up to the authors to convince the
reviewers that appropriate practices were followed to minimize
possible harm and that any harm caused by the work is greatly
outweighed by its benefits. The review process will be carried out in
two phases and authors will have an opportunity to provide a
length-limited response to the first-phase reviews.

\subsection{Paper Format}

Submissions must be single PDF files containing at most 12 pages in
the required new ACM format (see
\url{https://www.sigsac.org/ccs2017/format} for details and templates,
which you have presumably found if you are reading this!) of body
content, with any number of additional pages for the bibliography,
well-marked appendices, and any desired supplementary material.  When
relevant, submitters may include reviews from past submissions and
responses to them in the supplementary material.

Reviewers are not required to consider the appendices or supplementary
material, however, so submissions need to be intelligible and
convincing without them.  Submissions not meeting these guidelines, or
playing games to work around page limits, will be rejected by the PC
chairs without review.  In particular, papers should not use squeezing
tricks to adjust the (already very dense) ACM paper format, and moving
discussion of key related work or important definitions to appendices
may be grounds for rejection.

\subsection{Practice Talks}

Following the lead of USENIX Enigma, we want to improve the quality of
the conference and provide a better experience for both presenters and
attendees by holding practice sessions before the conference (see
\url{https://www.sigsac.org/ccs2017/practicefaq}). Presenting authors
of accepted papers are expected to participate in an on-line practice
session approximately three weeks before the conference.

\subsection{Conflicts of Interest}

The conference requires cooperation from both authors and program
committee members to ensure a process that is both fair in practice
and perceived to be fair by everyone. When submitting a paper, authors
are required to identify members of the program committee who may not
be able to provide an unbiased review.  This includes people with
strong personal or professional relationships such as advisor/advisee,
members of the same organization, and close collaborators (for
example, recent or repeated co-authors). In general, this means anyone
who a reasonable person with all the relevant information would
question as an impartial reviewer. The program co-chairs reserve the
right to request a more specific description of a conflict-of-interest
declaration from authors.

Program committee members who have a conflict of interest with a
paper, including program co-chairs, will be excluded from evaluation
and discussion of the paper, but because submissions are anonymous to
reviewers it is important for submitting authors to identify these
conflicts. In the case of a program co-chair, the other co-chairs who
do not have conflicts will be responsible for managing that paper.
Program co-chairs are not permitted to be involved as co-authors in
any submissions.




==> sec/Abandoned/Attacker_s_Analysis.tex <==
\subsection{Attacker's revenue}
We assume that attacker may choose three strategies: 1. Selfish Mining, 2. PSM and 3. Honest Mining. They can choose the most profitable way to mine. Here, what we are interested is in what condition the PSM can be the most profit strategy.

To answer the problem, first we need to maximize the reward of PSM strategy. To be specific, it needs to solve the following problem:

\textbf{(Problem 1)} Attacker revenue maximization: With given $\alpha_A$, $\alpha_i$ and $\gamma$, attacker revenue maximization is to maximize the attacker's revenue $R_A^S$ by choosing appropriate $T_L$ and $T_R$. This problem can be formally formulated as: 
\begin{subequations}\label{eq:atk1}
	\begin{align}
		  & \underset{T_R,T_L}{\text{Maximize}} &&  R_A^S,  \\ 
		 & \text{s.t.} && \alpha_A+\alpha_i+\alpha_h=1,\\ & &&
		 \alpha_A+\alpha_R=1,\\ & && 
		\alpha_A<0.5,\\ & && 0<\gamma<1.
	\end{align}
\end{subequations}

Assuming that the attacker can get the specific $\alpha_A$, $\alpha_i$ and $\gamma$, then we can get the attacker's revenue is maximized when:
\begin{equation}
\begin{aligned}
    &P(T_R)=((\alpha_A^2-2*\alpha_A+1)*\gamma-2*\alpha_A^2+3*\alpha_A-1)/
    \\&((\alpha_i^2+(2*\alpha_A-2)*\alpha_i+\alpha_A^2-2*\alpha_A+1)*\gamma
    \\&-\alpha_i^2+(2-3*\alpha_A)*\alpha_i-2*\alpha_A^2+3*\alpha_A-1)
    \end{aligned}
\end{equation}

\begin{equation}
    P(T_L)=1.
\end{equation}

Note that $P(T_L)\rightarrow 1$ means $T_L\rightarrow +\infty$. From the previous equation, we can draw the conclusion that to get the maximized revenue, attacker need to keep $T_L$ as long as possible. But there is no one-size-fits-all strategy for choosing $T_R$. It depends on the $\alpha_A$, $\alpha_i$ and $\gamma$.


==> sec/Abandoned/Block_sharing.tex <==
\section{Appendix: Block Sharing Strategy}
\label{sec:BlockSharing}
Before the exchange starts, the attacker can deploy a smart contract as an arbiter. Then, the attacker and the miner achieve a fair exchange of the partial block data through a simple interaction:

\begin{enumerate}
    \item The attacker generates a random key $k$ and encrypts the $b$ value with $k$, i.e., $\hat{b}=\mathsf{Enc}(b,k)$. Next, it computes the hash of $k$ $h_k\leftarrow H(k)$ and generates a proof:
    \begin{small}
    \begin{equation}
        \pi_e\overset{\rm R}\leftarrow\mathsf{Prove}((\hat{b},h, h_k),(b,k,nonce,r))
    \end{equation}
    \end{small}
    to prove the following relation:
    \begin{small}
    \begin{equation}
    \begin{aligned}
        H(b,nonce,r)=h\ \land\ 0 & \leq {\rm nonce}\leq2^{32}-1\\
        \land\ \hat{b}=\mathsf{Enc}(b,k) & \land h_k=H(k)
    \end{aligned}
    \end{equation}
    \end{small}
    is satisfied. Finally, it sends the tuple $(\pi_e,\hat{b},h,h_k)$ to the miner.
    \item After receiving the tuple $(\pi_e,\hat{b},h,h_k)$ from the attacker, the miner can verify whether $\pi_e$ is valid by computing $b\leftarrow\mathsf{Verify}((\hat{b},h, h_k),\pi_e)$. If $b=1$, the miner deposits to the arbiter contract the payment agreed upon by both parties beforehand, as well as the hash $h_k$.
    \item  The attacker checks whether the $h_k$ provided by the miner is valid, and the payment deposited is as previously agreed. If so, the attacker sends the key $k$ to the arbiter contract.
    \item The arbiter contract verifies that $h_k=H(k)$ holds. If it is the case, the contract transfers the payment to the attacker, otherwise it returns the payment to the miner. Since the $k$ disclosed to the contract will also be available to the miner at the same time, the miner can decrypt $\hat{b}$ by $b\leftarrow\mathsf{Dec}(\hat{b},k)$.
\end{enumerate}

Any miner as a buyer cannot obtain any information about $b$ without completing the payment. Meanwhile, any attacker acting as a seller cannot cheat the payment by submitting the wrong $b$. In this way, the attacker is able to sell the partial block data $b$ to a specific miner and gain revenue.

==> sec/Abandoned/Evaluation.tex <==

\section{Evaluation}
\label{sec:Eval}
This section uses numeric simulations to illustrate the mining strategy selection mechanism. Specifically, we considered two partial block data sharing strategies: full network sharing and partial network sharing. Full network sharing means the attacker sends the partial block information to all the miners in the network, and partial network sharing means only part of the miners in the network get the attacker's partial block data.

\subsection{Full Network Sharing}

To evaluate the effectiveness of the mining strategy selection mechanism, We first simulate the attacker with different mining power $\alpha_A$ and different network conditions $\gamma$. In this part, we assume that the attacker's partial block data can reach all the miners in the blockchain system, and all the miners in the mining pool are honest but greedy. That means any miner $i$ will surely participate in the attacker's private branch if its mining power $\alpha_i<\alpha_T$(See section~\ref{sec:Observation} for details). The simulation result is shown in figure~\ref{fig:MethodComp}. 

According to figure~\ref{fig:MethodComp}, when the attacker's mining power and the network condition are both relatively low, then honest mining is the best choice. But if the mining power is relatively higher, then the PSM strategy is more profitable. In Ethereum, the threshold value is 0.22, which means if the attacker controls more than $22\%$ mining power in Ethereum, it can launch the PSM and get extra revenue. According to~\cite{etherscan.io}, the largest mining pool in Ethereum controls more than 28\% of the mining power. 

If the attacker has a not-to-bad network condition, then the mining power requirement of PSM could be further reduced. If the attacker could assure more than $30\%$ of the honest miner can choose to mine its private branch when race occurs, PSM is always profitable regardless of the mining power.

To further illustrate the impact of $\alpha_A$ and $\gamma$ on $\alpha_i$, we simulate the changes of $\alpha_i$ when $\gamma$ and $\alpha_A$ take different values. The result is shown in figure~\ref{fig:MaxAi}. From the figure~\ref{fig:MaxAi}, we can see that the value of $\gamma$ has a significant impact on the greedy miner's decision. If the attacker can promise a $\gamma = 0.25$, then more than $70\%$ of the miners can get a higher reward in the attacker's private chain. Even if the $\gamma =0$, if the attacker's mining power is larger than 0.1, miners with more than $50\%$ mining power can get higher rewards in the attacker's private chain. And if the attacker's mining power is more than $22\%$, then joining the attacker's private branch is more profitable for all the miners.

\begin{figure*} \centering    
\subfigure[] {
 \label{fig:MethodComp}     
\includegraphics[width=\columnwidth]{fig/MethodComp.png}  
}     
\subfigure[] { 
\label{fig:MaxAi}     
\includegraphics[width=\columnwidth]{fig/MaxAi.png}     
}    

\caption{ (a) The most porfitable mining strategies for miner with different $\alpha_A$ and $\gamma$ (b) The changes of $\alpha_i$ when $\gamma$ and $\alpha_A$ take different values.}     
\label{fig}     
\end{figure*}
\subsection{Partial Network Sharing}

According to~\cite{capitalcounselor.com}, there are more than 1,000,000 Bitcoin miners with different education and cultural background in the world. Thus, it is not realistic to send the partial block to all of these miners and make them understand the meaning of these actions. In this section, we evaluate the performance of PSM when only part of the miners receives the partial block data.


\begin{figure*}[htbp]
\label{fig:partialshare}
	\centering
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 0.1]{\label{1B01}\includegraphics[width=5.5cm]{fig/MAi01.png}}
	\quad
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 0.3]{\label{1B015}\includegraphics[width=5.5cm]{fig/MAi03.png}}
	\quad
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 0.5]{\label{1B02}\includegraphics[width=5.5cm]{fig/MAi05.png}}
	\quad
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 0.7]{\label{2B01}\includegraphics[width=5.5cm]{fig/MAi07.png}}
	\quad
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 0.9]{\label{2B015}\includegraphics[width=5.5cm]{fig/MAi09.png}}
	\quad
	\subfigure[Greedy miners' maximum mining power $\alpha$ = 1.0]{\label{2B02}\includegraphics[width=5.5cm]{fig/MAi10.png}}
	\caption{The most profitable mining strategy for attacker when the partial block data can reach different amount of greedy miners}
	
\end{figure*}

The simulation result is shown in figure~\ref{fig:partialshare}. When the greedy miner's mining power is relatively small, the attacker is less likely to get more profit than honest mining, especially when its mining power is small. But when the attacker's mining power is large (more than 0.45), the PSM strategy is more likely to be more profitable than selfish mining. That is because when the attacker's mining power is large, fewer greedy miner means the attacker can share more rewards on its private branch. When the partial block data can reach half of the miners, the attacker with the PSM strategy can get more rewards than honest mining. But if the attacker's mining power is less than 0.22, then honest mining is still likely to be its best choice. For attacker with less than 0.1 mining power to get more profit with PSM, it needs to assure more than $70\%$ of the miners receive the partial block data, together with $\gamma>0.5$.







==> sec/Abandoned/Observation.tex <==

\section{Observation}\label{sec:Observation}

This section analyzes the combination of different mining strategies with numerical analysis to get the most profitable mining strategies for attackers with different mining power. Then we further investigate several detailed problems.

\subsection{For miners, which strategies can earn more revenue}

For miners, they can choose to mine on the attacker's private branch to get higher rewards. We are interested in what strategies can maximize the miner's profit with different mining power given $r$ $T_R$ and $\alpha_A$. 


In State 2, if miners choose the greedy strategy and participate in the private branch, then the revenue is:

\begin{equation}
\begin{aligned}
&R_i^G =\frac{\alpha_i}{\alpha_R} \times (\gamma  \alpha_R^2  P(T_L )+2 (1-\gamma )\alpha_R^2  P(T_L )+\\
&(1-\alpha_R  P(T_L )-\alpha_A  P(T_L ))\alpha_R )
\end{aligned}
\end{equation}.

If they choose the honest strategy, then the revenue is:

\begin{equation}
\begin{aligned}
&R_i^H =\alpha_i  P(T_L )+\alpha_h  P(T_L ) \alpha_i+\\
&(1-\alpha_hP(T_L )-\alpha_A  P(T_L )-\alpha_i P(T_L)) \alpha_i
\end{aligned}
\end{equation}.

The expected RER of a miner is
\begin{equation}
    RER_{Miner}=\frac{2-\alpha_A-\alpha_i}{(1-\alpha_A )(2-\gamma)}-1.
\end{equation}

$RER_{Miner}>0$ means taking part in the private branch is more profitable for the miners. In this condition, we have
\begin{equation}\label{equ:RERMiner}
\begin{aligned}
    \frac{2-\alpha_A-\alpha_i}{(1-\alpha_A )(2-\gamma)}-1>&0\\
    \alpha_i<\gamma+(1-\gamma)&\alpha_A
    \end{aligned}
\end{equation}

Let the mining power threshold $\alpha_T=\gamma+(1-\gamma)\alpha_A$, then $\alpha_i<\alpha_T$ means for miner $i$, joining the attacker's private branch is more profitable. 

From equation(\ref{equ:RERMiner}), we can see that the miner's RER mainly depends on $\gamma$ and $\alpha_A$. In theory, some researchers consider $\gamma=0.5$ in their works, and Ethereum even takes measures to fix $\gamma=0.5$. Since we assume the computational power of each miner/pool should be less than 0.5, $\gamma=0.5$ means mining on the attacker's private branch is always more profitable for the miners. 

If the $\gamma =0$, assuming a miner $k$ with mining power $\alpha_k$, it will join the attacker's private branch only if $\alpha_k<\alpha_A$.  

But in practice, on the one hand, since the attacker broadcasts the private branch information to miners, other miners may refuse to mine on the malicious private chain when racing occurs. This will make the $\gamma = 0$. On the other hand, it is possible that not all the miners will receive the attacker's message, and only part of the miners can have the chance to join the private branch.


\subsection{How to get $\alpha_i$ when $\gamma =0$}

According to equation(\ref{equ:RERMiner}), when $\gamma =0$, assuming the mining power of miner k is $\alpha_k$, it is more profitable for miners to join the attacker's private branch when $\alpha_k<\alpha_A$. According to~\cite{etherscan.io}, we show the top 25 miners mining power in figure~\ref{fig:TopMiner}.
\begin{figure}[htbp]
	\centerline{\includegraphics[width=0.8\columnwidth]{fig/TopMiners.png}}
	\caption{Mining power distibution in Ethereum}
	\label{fig:TopMiner}
\end{figure}

From the figure~\ref{fig:TopMiner}, we can see that if the attacker's mining power is larger than $1\%$, then miners with more than $9\%$ mining power will tend to join the attacker's branch. If the attacker's mining power is larger than $2\%$, then miners with more than $18\%$ mining power will work on the attacker's branch. %In the following experiment, we calculate the $\alpha_i$ based on the data in~\cite{etherscan.io}.

\subsection{For the attacker, how to choose $T_L$ and $T_R$ can get the most revenue?}

We assume that the attacker may choose three strategies: 1. selfish Mining, 2. PSM, and 3. honest mining. Here, we are interested in what strategies can maximize the attacker's revenue.

To answer the problem, first, we need to figure out how to choose $T_L$, and $T_R$ can maximize the reward of attacker. To be specific, it needs to solve the following problem:

\textbf{(Problem)} Attacker revenue maximization: With given $\alpha_A$, $\alpha_i$ and $\gamma$, attacker revenue maximization is to maximize the attacker's revenue $R_A^S$ by choosing appropriate $T_L$ and $T_R$. This problem can be formally formulated as: 
\begin{subequations}\label{eq:atk1}
	\begin{align}
		  & \underset{T_R,T_L}{\text{Maximize}} &&  R_A^S,  \\ 
		 & \text{s.t.} && \alpha_A+\alpha_i+\alpha_h=1,\\ & &&
		 \alpha_A+\alpha_R=1,\\ & && 
		\alpha_A<0.5,\\ & && 0<\gamma<1.
	\end{align}
\end{subequations}
To solve the problem, first taking the partial derivatives with respect to $T_L$ and $T_R$ respectively, let $dT_L$ be the partial derivative of $R_A^S$ with respect to $T_L$, and $dT_R$ be the partial derivative of $R_A^S$ with respect to $T_R$, we can get:
\begin{equation}
\begin{aligned}
    dT_L=&(((-\alpha_i^2)+(2-2\alpha_A)\alpha_i-\alpha_A^2+2\alpha_A-1)\gamma+\\
    &\alpha_i^2+(3\alpha_A-2)\alpha_i+2\alpha_A^2-3\alpha_A+1)P(T_R)+\\
    &(\alpha_i^2+(2\alpha_A-2)\alpha_i+\alpha_A^2-2\alpha_A+1)\gamma-\\
    &\alpha_i^2+(2-3\alpha_A)\alpha_i-2\alpha_A^2+3\alpha_A-1,
    \end{aligned}
\end{equation}
\begin{equation}
\begin{aligned}
    dT_R=&(((-\alpha_i^2)+(2-2\alpha_A)\alpha_i-\alpha_A^2+2\alpha_A-1)\gamma+\\
    &\alpha_i^2+(3\alpha_A-2)\alpha_i+2\alpha_A^2-3\alpha_A+1)P(T_L)+\\
    &(\alpha_A^2-2\alpha_A+1)\gamma-2\alpha_A^2+3\alpha_A-1
    \end{aligned}
\end{equation}

Let $dT_L=0$, then we can get $P(T_R)=1$. That means $R_A^S$ is monotonic when $P(T_R)\in [0,1)$. Take any $T_R\leq 0$, if $dT_L>0$, means PSM is more profitable than honest mining, but it still need to calculate the value of $dT_R$ to see if the PSM is the most profitable strategy. If $dT_L<0$, means attacker should not spend any time on PSM, $T_L=0$.

With $T_L=0$, we can get the value of $dT_R$. If $dT_R>0$ means the original selfish mining is the most profitable strategy. If $dT_R<0$ and $dT_L>0$ means the PSM is the most profitable strategy. Otherwise, attacker should choose honest mining.




\nop{\subsection{For Attacker, How to choose the $T_R$}

In PSM, to secure the mining reward of the participants, attacker needs to have a clear statements about in what condition the private branch will be released. 

For the greedy miner choose to mine on the attacker's private branch, 

For attacker, it need to carefully choose the mining time $T_R$. If the $T_R$ is not long enough, then the private branch may be released prematurely. If the value of $T_R$ is too large, then racing with the public branch is more likely to occur. To be specific, it needs to solve the following problem:

\textbf{(Problem 1)} Attacker revenue maximization: With given $\alpha_A$, $\alpha_i$ and $\gamma$, attacker revenue maximization is to maximize the attacker's revenue $R_A^S$ by choosing appropriate $T_L$. This problem can be formally formulated as: 
\begin{subequations}\label{eq:atk1}
	\begin{align}
		  & \underset{T_L}{\text{Maximize}} &&  R_A^S,  \\ 
		 & \text{s.t.} && \alpha_A+\alpha_i+\alpha_h=1,\\ & &&
		 \alpha_A+\alpha_R=1,\\ & && 
		\alpha_A<0.5,\\ & && 0<\gamma<1.
	\end{align}
\end{subequations}

By deriving the $R_A^S$, we have:
\begin{equation}
   R_A^S'= \alpha_h^2\times\gamma+\alpha_h\times\alpha_i+(2\times\alpha_A-1)\times\alpha_h
\end{equation}
}
